Curved patch mapping and tracking for irregular terrain modeling: Application to bipedal robot foot placement

Legged robots need to make contact with irregular surfaces, when operating in unstructured natural terrains. Representing and perceiving these areas to reason about potential contact between a robot and its surrounding environment, is still largely an open problem. This paper introduces a new framework to model and map local rough terrain surfaces, for tasks such as bipedal robot foot placement. The system operates in real-time, on data from an RGB-D and an IMU sensor. We introduce a set of parametrized patch models and an algorithm to fit them in the environment. Potential contacts are identified as bounded curved patches of approximately the same size as the robot's foot sole. This includes sparse seed point sampling, point cloud neighborhood search, and patch fitting and validation. We also present a mapping and tracking system, where patches are maintained in a local spatial map around the robot as it moves. A bio-inspired sampling algorithm is introduced for finding salient contacts. We include a dense volumetric fusion layer for spatiotemporally tracking, using multiple depth data to reconstruct a local point cloud. We present experimental results on a mini-biped robot that performs foot placements on rocks, implementing a 3D foothold perception system, that uses the developed patch mapping and tracking framework.

==> bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/bio/kanoulas_new.jpg}}]{Dimitrios Kanoulas}
is a senior postdoctoral researcher at the Humanoids and Human-Centered Mechatronics Lab at the Istituto Italiano di Tecnologia (IIT), working with Dr. Nikos Tsagarakis and Prof. Darwin Caldwell on the WALK-MAN, CENTAURO, and CogIMon European projects.  He was the perception team leader during the DARPA Robotics Challenge 2015.  In August 2014, he completed his Ph.D. at the Geometric and Physical Computing Lab in the College of Computer and Information Science at Northeastern University, advised by Prof. Marsette Vona.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/bio/tsagarakis.pdf}}]{Nikos G. Tsagarakis}
received his D.Eng. degree in Electrical and Computer Science Engineering in 1995 from the Polytechnic School of Aristotle University, Greece, his M.Sc. degree in Control Engineering in 1997 and his Ph.D. in Robotics from the University of Salford, UK, in 2000.  He is Tenured Senior Scientist at IIT with overall responsibility for Humanoid design $\&$ Human Centred Mechatronics development.  Since 2013, he is also serving as a Visiting Professor at the Centre for Robotics Research (CORE), Department of Informatics, King’s College University, London, UK.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/bio/vona.jpg}}]{Marsette Vona}
completed his B.A. at Dartmouth College in 1999 and his M.S. and Ph.D. in EECS at MIT in 2001 and 2009.  He spent 2001-2003 at NASA/JPL building 3D user interfaces for the Mars Exploration Rover mission, for which he was a recipient of the NASA Software of the Year award in 2004.  In 2010, he joined the faculty at the College of Computer and Information Science at Northeastern University as Assistant Professor.  He founded the Geometric and Physical Computing group and received the NSF CAREER award to study 3D perception and compliant contact.  In 2015 he returned to JPL to work full time on software for designing and operating NASA missions.
\end{IEEEbiography}
